CLIP the Gap: A Single Domain Generalization Approach for Object Detection

Single Domain Generalization (SDG) tackles the problem of training a model on a single source domain so that it generalizes to any unseen target domain. While this has been well studied for image classification, the literature on SDG object detection remains almost non-existent. To address the challenges of simultaneously learning robust object localization and representation, we propose to leverage a pre-trained vision-language model to introduce semantic domain concepts via textual prompts. We achieve this via a semantic augmentation strategy acting on the features extracted by the detector backbone, as well as a text-based classification loss. Our experiments evidence the benefits of our approach, outperforming by 10% the only existing SDG object detection method, Single-DGOD [49], on their own diverse weather-driving benchmark.

==> tables/class_results_day_clear.tex <==
\begin{table}[h]
 
    \begin{center}
     \renewcommand{\arraystretch}{1.2}
    \resizebox{\linewidth}{!}{
    \setlength{\tabcolsep}{3pt}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{r | c c c c c c c  c } \toprule
    \multicolumn{1}{c}{} & \multicolumn{7}{c}{AP} & mAP \\ \cmidrule(lr{.75em}){2-8}
     \multicolumn{1}{c}{Method} & Bus  & Bike & Car & Motor & Person & Rider & Truck & All  \\
    F. R-CNN~\cite{ren2016faster} &  50.2 & 42.4 & 65.7 & 41.9 & 44.8 & 40.0 & 51.9 & 48.1  \\
    % SW \cite{pan2019switchable} & - & - & - & - & - & - & - & - \\
    % IBN-Net \cite{pan2018two} & - & - & - & - & - & - & - & - \\
    % IterNorm \cite{huang2019iterative} & - & - & - & - & - & - & - & - \\
    % ISW \cite{choi2021robustnet} & - & - & - & - & - & - & - & - \\
    S-DGOD \cite{wu2022single} & \textbf{68.8} & \textbf{50.9} & 53.9 & \textbf{56.2} & 41.8 & \textbf{52.4} & \textbf{68.7} & \textbf{56.1} \\
    \hline
    Ours & 54.9 & 46.2 & \textbf{66.1} & 45.2 & \textbf{47.5} & 44.6 & 54.3 & 51.3 \\
    \bottomrule
    \end{tabular}
    }
    \end{center}
    \caption{\textbf{Day clear per class results} .
    } 
    \label{tab:class_day_clear}
\end{table}


